Self-Refinement of Language Models from External Proxy Metrics Feedback

It is often desirable for Large Language Models (LLMs) to capture multiple objectives when providing a response. In document-grounded response generation, for example, agent responses are expected to be relevant to a user's query while also being grounded in a given document. In this paper, we introduce Proxy Metric-based Self-Refinement (ProMiSe), which enables an LLM to refine its own initial response along key dimensions of quality guided by external metrics feedback, yielding an overall better final response. ProMiSe leverages feedback on response quality through principle-specific proxy metrics, and iteratively refines its response one principle at a time. We apply ProMiSe to open source language models Flan-T5-XXL and Llama-2-13B-Chat, to evaluate its performance on document-grounded question answering datasets, MultiDoc2Dial and QuAC, demonstrating that self-refinement improves response quality. We further show that fine-tuning Llama-2-13B-Chat on the synthetic dialogue data generated by ProMiSe yields significant performance improvements over the zero-shot baseline as well as a supervised fine-tuned model on human annotated data.

==> inference_table.tex <==
\begin{table*}[h]
\label{sample-table}
\vskip 0.15in
\begin{center}
%\begin{scriptsize}
%\begin{footnotesize}
\begin{footnotescript}
\begin{sc}
\begin{tabular}{lccccccr}
\toprule
 Initial Exemplars + Metrics & Stage & Rouge-L & BERT-Recall & BERT K-Prec. & Recall & K-Prec. \\
\midrule
 Flan-T5-XXL (11B) Results & & & & & & \\
\midrule
 3-Shot / Only Rou-L + Rou-1 & Initial & 21.50 & 27.27 & 38.08 & 31.19 & 75.58 \\
 & Final & 21.84 & 28.96 & 41.41 & 33.96 & 78.78 \\
\hline
 0-Shot / Only Rou-L + Rou-1 & Initial & 21.55 & 28.11 & 40.42 & 32.34 & 76.77 \\
& Final & 21.72 & 29.29 & 42.74 & 34.14 & 79.29 \\
\hline
 3-Shot / Only RM & Initial & 22.67 & 28.80 & 42.83 & 33.00 & 80.42\\
 & Final & 22.65 & 28.91 & 43.55 & 33.31 & 81.14 \\
 \hline
  0-Shot / Only RM & Initial & 22.33 & 28.91 & 44.58 & 33.61 & 81.29\\
 & Final & 22.43 & 29.17 & 45.60 & 34.20 & 82.25 \\
 \hline
 3-Shot / Rou + RM    & Initial & 22.61 & 28.75 & 42.60 &  32.75 & 80.36    \\
 & Final & \textbf{22.71} & 29.89 & 44.86 & 34.76 & 81.98\\
\hline
 0-Shot / Rou + RM   & Initial & 22.30 & 28.94 & 44.55 &  33.68 & 81.56    \\
& Final & 22.38 & \textbf{30.10} & \textbf{46.60} & \textbf{35.58} & \textbf{83.13}\\
\hline\midrule
Llama-2-13B-Chat Results & & & & & & \\
\midrule
 3-Shot / Only Rou-L + Rou-1 & Initial & 20.63 & 29.35 & 34.32 & 36.49 & 71.03 \\
& Final & 20.23 & 30.22 & 36.07 & 38.82 & 72.74        \\
\hline
 0-Shot / Only Rou-L + Rou-1 & Initial & 19.31 & 28.92 & 34.44 & 38.45 & 70.33 \\
 & Final & 18.95 & 29.67 & 36.04 & 40.43 & 71.76        \\
\hline
 3-Shot / Only RM & Initial & \textbf{21.50} & 30.35 & 39.20 & 36.89 & 76.29 \\
& Final & 21.25 & 30.11 & 39.51 & 36.85 & 76.53 \\
\hline
 0-Shot / Only RM & Initial & 19.97 & 29.65 & 34.33 & 38.07 & 70.08 \\
& Final & 19.95 & 29.89 & 40.68 & 38.59 & 76.73 \\
\hline
 3-Shot / Rou + RM & Initial & 21.48 & 30.29 & 39.15 & 36.79 & 76.34 \\
& Final & 21.11 & \textbf{30.95} & 40.05 & 38.62 & 76.89 \\
\hline
 0-Shot / Rou + RM & Initial & 20.36 & 30.17 & 40.68 & 38.59 & 76.84 \\
& Final & 20.06 & 30.64 & \textbf{41.46} & \textbf{40.00} & \textbf{77.43} \\
\bottomrule
\end{tabular}
\end{sc}
%\end{scriptsize}    
%\end{footnotesize}
\end{footnotescript}
\end{center}
\vskip -0.1in
\caption{Experimental Results on MultiDoc2Dial test set, containing 10,204 instances. Experiments are reported with the Flan-T5-XXL and Llama-2-13B-Chat models, using 3 Rouge (ROU) measures, the WeCheck reward model (abbreviated as RM), and both in tandem for sufficiency thresholding. "Initial" refers to scoring of the generations after rejection sampling, while "Final" includes both initial generations that cleared the threshold and refined responses after the refinement loop. In thresholding, Rouge-L refers to computing said score between the candidate response with both the grounding document and the given user query, and Rouge-1 is with respect to the document; "Rouge" refers to all 3 of these metrics together. Highest scores are boldfaced for each model.
}

\end{table*}

==> quactable.tex <==
\begin{table*}[t]
\label{sample-table}
\vskip 0.15in
\begin{center}
%\begin{scriptsize}
%\begin{footnotesize}
\begin{footnotescript}
\begin{sc}
\begin{tabular}{lccccccr}
\toprule
 Initial Exemplars + Metrics & Stage & Rouge-L & BERT-Recall & BERT K-Prec. & Recall & K-Prec. \\
\midrule
Flan-T5-XXL (11B) Results & & & & & & \\
\midrule
 0-Shot / Only Rou-L + Rou-1 & Initial & \textbf{41.57} & 40.70 & 43.31 & 44.87 & 87.57 \\
& Final & 40.00 & \textbf{41.47} & 46.06 & \textbf{45.77} & 88.26 \\
\hline
  0-Shot / Only RM & Initial & 37.01 & 36.58 & 48.82 & 40.21 & 91.51\\
 & Final & 34.99 & 35.00 & 49.69 & 38.61 & 91.58 \\
 \hline
 0-Shot / Rou + RM   & Initial & 38.20 & 37.28 & 48.44 &  40.78 & 91.38    \\
& Final & 35.85 & 37.13 & \textbf{50.91} & 41.21 & \textbf{91.89} \\
\hline\midrule
Llama-2-13B-Chat Results & & & & & & \\
\midrule
 0-Shot / Only Rou-L + Rou-1 & Initial & \textbf{31.36} & 35.12 & 40.79 & 42.86 & 83.08 \\
 & Final & 29.23 & \textbf{35.28} & 42.87 & \textbf{43.63} & 82.96       \\
\hline
 0-Shot / Only RM & Initial & 29.83 & 33.11 & 46.64 & 39.22 & 87.78 \\
& Final & 28.70 & 31.83 & 47.79 & 37.62 & 87.24 \\
\hline
 0-Shot / Rou + RM & Initial & 28.85 & 32.29 & 46.59 & 38.54 & 88.04 \\
& Final & 26.76 & 32.39 & \textbf{48.05} & 39.64 & \textbf{88.11} \\
\bottomrule
\end{tabular}
\end{sc}
%\end{scriptsize}    
%\end{footnotesize}
\end{footnotescript}
\end{center}
\vskip -0.1in
\caption{Experimental Results on QuAC test set (1,000 instances). Experiments are reported with the Flan-T5-XXL and Llama-2-13B-Chat models with \textsc{0-shot} initial exemplars. Highest scores are boldfaced for each model.}
\end{table*}

==> relatedwork.tex <==
\section{Related Work}
There have been numerous work on self-refine, often dubbed as self-critique, self-improve, etc. According to \cite{huang2023large}, a critical distinction lies in the source of the feedback \cite{pan2023}. Internal feedback relies on the model's inherent knowledge and parameters to reassess its outputs. External feedback incorporates inputs from humans, other models. Our work is inspired by \cite{madaan2023selfrefine}, an approach for improving initial outputs from LLMs through iterative feedback and refinement. Unlike \citet{madaan2023selfrefine}, however, who rely on very large LLMs (GPT-3.5, ChatGPT, GPT-4) as the source of \textit{internal} feedback, we introduce \textit{external} feedback with proxy metrics and enable self-refinement technique to work with relatively weaker LLMs including Flan-T5-XXL and LlaMA-2-13B-Chat in content-grounded setups. We largely attribute the success of our technique to the fact that we rely on the grounding documents as the proxy reference for external metrics feedback.

\cite{wang2023shepherd} propose Shepherd with internal feedback, a language model tuned to critique its own responses and suggest refinements, extending beyond the capabilities of an untuned model to identify diverse errors and provide suggestions to remedy them. \cite{paul2023refiner} propose \textsc{refiner}, a framework for finetuning LMs to explicitly generate intermediate reasoning steps while interacting with a critic model that provides automated feedback on the reasoning. 

\cite{gou2023tool} proposes \textsc{critic} that interacts with appropriate tools, e.g. calculator, search engine, wikipedia, knowledge base, code interpreter, text APIs, to evaluate certain aspects of the text and then revises the output based on the feedback obtained during the validation process. \cite{chen2023selfdebug} propose Self-Debugging, which teaches a large language model to debug its predicted program via few-shot demonstrations. \cite{olausson2024selfrepair} critically examines the LLM's ability to perform self-repair on problems taken from HumanEval and APPS and concludes that self-repair still lags behind what can be achieved with human-level debugging. \cite{gao2023acl} propose RARR (Retrofit Attribution using Research and Revision) that revises a generated text on the basis of the relevant evidence retrieved by re-search.
 
%external tools and knowledge sources (Gou et al, 2023; Chen et al., 2023b; Olausson et al., 2023; Gao et al., 2023)



==> self-refinement-algo.tex <==
\begin{figure*}[t]
{\centering
\begin{minipage}{0.7\linewidth}
\begin{algorithm}[H]
\small
\caption{\hspace{-1mm}\textbf{:} \textit{Self-Refinement} Algorithm}

\SetKwInOut{Input}{Input}
\SetKwInOut{Begin}{Begin}
\SetKwInOut{Output}{output}

\label{alg:cap}
\begin{algorithmic}[1]
\hspace{-7mm}

\Input{~Model} $\mathcal{M}$; \newline
$x$ \hspace{-1.5mm} \colon \mbox{Task Input (document, context, $\dots$)}
\newline
\mathcal{P} \colon \mbox{User-defined set of principles} \newline
\mathcal{T} \colon \mbox{Set of metrics corresponding to $\mathcal{P}$. %Note $|\mathcal{T}| \geq |\mathcal{P}|$
} 
\newline
i \colon \mbox{Initial generation prompt}\newline
r_p \colon \hspace{1mm} \mbox{Refinement prompt for principle $p$} \newline
\tau = [\tau_1, \tau_2, \dots, \tau_k] \colon \mbox{Output quality metric i has threshold $\tau_i$} \newline 
w = [w_1, w_2, \dots, w_k] \colon \mbox{Quality metric i has weight $w_i$} \newline
\lambda \colon \mbox{Improvement threshold for weighted metric combination} \newline
{N} \colon \mbox{Number of initial responses generated per turn} \newline

\newline
\Begin{~}
\newline
\mathcal{Y}_0 = \{y_n\}_{n=1}^N \quad\mbox{with}\quad y_n \sim p_{\mathcal{M}}(y \mid x, i)\newline
y^0 = \arg\max_{y \in \mathcal{Y}_0}\left\{\sum_{t=1}^{|\mathcal{T}|} \mathbbm{1}(\arg\max_{y' \in \mathcal{Y}_0}\{m_t(y', x)\} = y) \right\}\newline
\newline
\textbf{if} \hspace{1mm} \sum_{t=1}^{|\mathcal{T}|} \mathbbm{1}(m_t(y^0, x)\geq \tau_t) = |\mathcal{T}|\hspace{-1mm}: \newline
\indent \textbf{return} \hspace{1mm} y_0 \newline
\textbf{else:} \newline
\indent \textbf{for} \hspace{1mm} iteration \hspace{1mm} j = 0, 1, \dots J: \newline   
\indent \indent \mathcal{Y}_{j+1} = \{y_p\}_{p=1}^{|\mathcal{P}|} \quad\mbox{with}\quad y_p \sim p_{\mathcal{M}}(y \mid y^j, x, r_p)\newline
\indent\indent y^{j+1} = \arg\max_{y \in \mathcal{Y}_{j+1}}\left\{\sum_{t=1}^{|\mathcal{T}|} \mathbbm{1}(\arg\max_{y' \in \mathcal{Y}_{j+1}}\{m_t(y', x)\} = y) \right\}\newline
\indent\indent \textbf{if} \hspace{1mm} \sum_{t=1}^{|\mathcal{T}|} \mathbbm{1}(m_t(y^{j+1}, x)\geq \tau_p) = |\mathcal{T}|\hspace{-1mm}: \newline
\indent\indent\indent \textbf{return} \hspace{1mm} y^{j+1} \newline
\indent\indent \textbf{else if} \hspace{1.5mm}\sum_{t=1}^{|\mathcal{T}|} w_t \cdot \mathbbm{1}(m_t(y^{j+1}, x) \geq m_t(y^{j}, x)) < \lambda \textbf{:} \newline
\indent\indent\indent y^{j+1} = y^j \newline
\indent\textbf{return} \hspace{1mm} y^J
%
\end{algorithmic}
\end{algorithm}
\end{minipage}
\par
\caption{Overview of the \_\_\_\_ algorithm. This incorporates: (i) Best-of-N (rejection) sampling with the initial generation prompt, (ii) determining the best initial response based on proxy metric feedback scores, and comparing it to a sufficiency threshold vector, (iii) accepting the response if sufficient or proceeding to refinement if insufficient, (iv) at each iteration, attempting to refine with respect to each principle and perform Best-of-N sampling on $|P|$ responses, (v) comparing the scores of the best refinement candidate against the threshold, and (vi) if still insufficient, using a weighted combination of metric indicators to determine improvement relative to the previous best response.}
}
\end{figure*}

